LiRCDepth: Lightweight Radar-Camera Depth Estimation via Knowledge Distillation and Uncertainty Guidance

Recently, radar-camera fusion algorithms have gained significant attention as radar sensors provide geometric information that complements the limitations of cameras. However, most existing radar-camera depth estimation algorithms focus solely on improving performance, often neglecting computational efficiency. To address this gap, we propose LiRCDepth, a lightweight radar-camera depth estimation model. We incorporate knowledge distillation to enhance the training process, transferring critical information from a complex teacher model to our lightweight student model in three key domains. Firstly, low-level and high-level features are transferred by incorporating pixel-wise and pair-wise distillation. Additionally, we introduce an uncertainty-aware inter-depth distillation loss to refine intermediate depth maps during decoding. Leveraging our proposed knowledge distillation scheme, the lightweight model achieves a 6.6% improvement in MAE on the nuScenes dataset compared to the model trained without distillation. Code: https://github.com/harborsarah/LiRCDepth

==> chapters/rebuttal.tex <==
% \vspace{-10mm} 
\begin{figure*}[t]
    \centering
    {\large \textbf{LiRCDepth: Lightweight Radar-Camera Depth Estimation via Knowledge Distillation and Uncertainty Guidance}}
% \vspace{-5mm}    
\end{figure*}

We sincerely appreciate the valuable feedback provided by the reviewers and are encouraged by their highly positive responses. It is gratifying to see our knowledge distillation pipeline and the uncertainty-rectified depth loss recognized as significant contributions. We have carefully considered all the reviewers' comments and are committed to incorporating their insights to further improve our work.

\textbf{Response to Reviewer \#2 (R2) }
The reviewer expressed interest in analyzing the results under different weather conditions. To address this, we evaluated our model's performance under three distinct scenarios: normal weather, rainy conditions, and night-time scenarios, presented in Table \ref{tab:normal}, Table \ref{tab:rain} and Table \ref{tab:night}, respectively. The nuScenes test set is split into 4,254 samples for normal weather, 900 samples for rainy conditions, and 704 samples for night-time. We compared the results of our proposed LiRCDepth (KD) model against CaFNet (T) and RadarNet. The findings are presented and discussed in detail below.
\begin{table}[ht]
\vspace{-1mm}
\centering
\caption{Performance Comparison on sub Test Set under Normal Weather.}
\vspace{-2mm}
\label{tab:normal}
\resizebox{8.5cm}{!} 
{
\centering

\begin{tabular}{c||c|cccccc}
\hline
\multirow{2}{*}{Eval Distance} & \multirow{2}{*}{Method}  & \multicolumn{6}{c}{Metrics} \\ \cline{3-8} 
                                    &          & MAE $\downarrow$ & RMSE $\downarrow$ & AbsRel $\downarrow$ & RMSElog $\downarrow$ & $\delta_{1}$ $\uparrow$& $\delta_{2}$ $\uparrow$   \\ \hline
\multirow{3}{*}{50m}                & RadarNet  \cite{radarnet} & 1.653 & 3.630 & 0.096 & 0.159 & 0.910 & 0.970  \\ 
                                    % \cline{2-8} 
                                    & CaFNet (T)~\cite{cafnet}  & 1.272 & 2.941 & 0.072 & 0.133 & 0.939&  0.978\\
                                    & LiRCDepth (KD) & 1.402& 3.107 &0.083 &0.142 &0.926 &0.974 \\

                                    
                                    \hline
\multirow{3}{*}{70m}                
                                    & RadarNet    \cite{radarnet} & 1.978 & 4.411 & 0.098 & 0.169 & 0.903 & 0.966     \\ 
                                    % \cline{2-8} 
                                    & CaFNet (T)~\cite{cafnet} & 1.569 & 3.706& 0.075&0.142 &0.932 &0.975 \\
                                    & LiRCDepth (KD) & 1.763& 4.036& 0.086& 0.153& 0.917& 0.970\\

                                    \hline
\multirow{3}{*}{80m}                & RadarNet   \cite{radarnet}  & 2.075 & 4.690 & 0.099 & 0.172 & 0.902& 0.965\\ 
                                    & CaFNet (T)~\cite{cafnet}   & 1.652&3.951 &0.076 &0.144 &0.930 & 0.975\\ 
                                    & LiRCDepth (KD) & 1.865 &4.339 &0.087 &0.156 &0.915 &0.969 \\

                                    \hline
\end{tabular}
}

\vspace{-3mm}
\end{table}

\begin{table}[ht]
\vspace{-1mm}
\centering
\caption{Performance Comparison on sub Test Set under Rainy Scenario.}
\vspace{-2mm}
\label{tab:rain}
\resizebox{8.5cm}{!} 
{
\centering

\begin{tabular}{c||c|cccccc}
\hline
\multirow{2}{*}{Eval Distance} & \multirow{2}{*}{Method}  & \multicolumn{6}{c}{Metrics} \\ \cline{3-8} 
                                    &          & MAE $\downarrow$ & RMSE $\downarrow$ & AbsRel $\downarrow$ & RMSElog $\downarrow$ & $\delta_{1}$ $\uparrow$& $\delta_{2}$ $\uparrow$   \\ \hline
\multirow{3}{*}{50m}                & RadarNet  \cite{radarnet} & 1.459 & 3.535 & 0.099 & 0.175 & 0.918 & 0.967 \\
                                    % \cline{2-8} 
                                    & CaFNet (T)~\cite{cafnet}  & 1.150 &2.960 &0.078 &0.152 &0.939 &0.975 \\
                                    & LiRCDepth (KD) &1.311 &3.153 &0.092 &0.164 &0.926 &0.970 \\
                                    
                                    \hline
\multirow{3}{*}{70m}                
                                    & RadarNet    \cite{radarnet} & 1.672 & 4.116 & 0.100 & 0.169 & 0.903 & 0.966 \\
                                    % \cline{2-8} 
                                    & CaFNet (T)~\cite{cafnet}   & 1.336& 3.503& 0.079& 0.157& 0.935& 0.974\\
                                    & LiRCDepth (KD) &1.555 &3.850 &0.094 &0.172 &0.921 &0.967 \\

                                    \hline
\multirow{3}{*}{80m}                & RadarNet   \cite{radarnet}  & 1.750 & 4.361 & 0.100 & 0.185 & 0.913 & 0.964 \\
                                    & CaFNet (T)~\cite{cafnet}  & 1.401& 3.692& 0.080& 0.158& 0.934& 0.973\\
                                    & LiRCDepth (KD) &1.645 &4.110 &0.095 &0.174 &0.919 &0.966 \\

                                    
                                    \hline
\end{tabular}
}
\vspace{-3mm}
\end{table}

\begin{table}[ht]
\vspace{-1mm}
\centering
\caption{Performance Comparison on sub Test Set under Night-time Scenario.}
\vspace{-2mm}
\label{tab:night}
\resizebox{8.5cm}{!} 
{
\centering

\begin{tabular}{c||c|cccccc}
\hline
\multirow{2}{*}{Eval Distance} & \multirow{2}{*}{Method}  & \multicolumn{6}{c}{Metrics} \\ \cline{3-8} 
                                    &          & MAE $\downarrow$ & RMSE $\downarrow$ & AbsRel $\downarrow$ & RMSElog $\downarrow$ & $\delta_{1}$ $\uparrow$& $\delta_{2}$ $\uparrow$   \\ \hline
\multirow{3}{*}{50m}                & RadarNet  \cite{radarnet} & 2.343 &4.686 &0.150 &0.235 &0.840 &0.935 \\
                                    % \cline{2-8} 
                                    & CaFNet (T)~\cite{cafnet}   & 2.158& 4.502& 0.123& 0.206& 0.872& 0.948\\
                                    & LiRCDepth (KD) &2.453 &4.907 &0.144 &0.225 &0.841 &0.935 \\

                                    
                                    \hline
\multirow{3}{*}{70m}                
                                    & RadarNet~\cite{radarnet}  & 2.865 & 5.937 & 0.154 & 0.251 & 0.830 & 0.928 \\
                                    % \cline{2-8} 
                                    & CaFNet (T)~\cite{cafnet}  &2.733 &5.812 &0.129 &0.221 &0.855 &0.940 \\
                                    & LiRCDepth (KD) & 3.154 &6.469 &0.152 &0.244 &0.819 &0.923 \\

                                    \hline
\multirow{3}{*}{80m}                & RadarNet   \cite{radarnet}  & 3.014 & 6.340 & 0.155 & 0.255 & 0.827 & 0.926 \\
                                    & CaFNet (T)~\cite{cafnet}  & 2.894& 6.225& 0.131& 0.225& 0.851&0.938 \\
                                    & LiRCDepth (KD) &3.344 &6.946 &0.154 &0.248 &0.814 &0.920 \\

                                    
                                    \hline
\end{tabular}
}
\vspace{-3mm}

\end{table}


As evident from the tables above, estimating depth during night-time poses significant challenges due to the reduced visibility and lack of reliable visual cues. In contrast, during rainy scenarios, the algorithms demonstrate the ability to predict reasonable depth values, leveraging the robustness of radar sensors. This highlights the importance of developing more robust depth estimation algorithms specifically designed for night-time conditions in future research.

\textbf{Future Works}


As recommended by reviewers R3, R5, and R6, we plan to explore the development of models with even lighter weights in the future. Additionally, we aim to evaluate our models on various datasets to further validate and demonstrate their effectiveness and generalizability.
